DONAPI: Malicious NPM Packages Detector using Behavior Sequence Knowledge Mapping

With the growing popularity of modularity in software development comes the rise of package managers and language ecosystems. Among them, npm stands out as the most extensive package manager, hosting more than 2 million third-party open-source packages that greatly simplify the process of building code. However, this openness also brings security risks, as evidenced by numerous package poisoning incidents. In this paper, we synchronize a local package cache containing more than 3.4 million packages in near real-time to give us access to more package code details. Further, we perform manual inspection and API call sequence analysis on packages collected from public datasets and security reports to build a hierarchical classification framework and behavioral knowledge base covering different sensitive behaviors. In addition, we propose the DONAPI, an automatic malicious npm packages detector that combines static and dynamic analysis. It makes preliminary judgments on the degree of maliciousness of packages by code reconstruction techniques and static analysis, extracts dynamic API call sequences to confirm and identify obfuscated content that static analysis can not handle alone, and finally tags malicious software packages based on the constructed behavior knowledge base. To date, we have identified and manually confirmed 325 malicious samples and discovered 2 unusual API calls and 246 API call sequences that have not appeared in known samples.

==> tables/KeyAPIs.tex <==
\begin{table*}[h]
\caption{The key APIs we monitor and their implementation files.}
\label{tab:KeyAPIs}
\resizebox{\linewidth}{!}{
\centering
% \setlength{\tabcolsep}{10pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1.5} % Default value: 1

\begin{tabular}{ll}
\toprule
\textbf{Files} & \textbf{APIs}\\
\midrule
./lib/fs.js & \makecell[l]{fs.access, fs.accessSync, fs.appendFile, fs.appendFileSync, fs.chmod, fs.chmodSync,\\ fs.chown, fs.chownSync, fs.createReadStream, fs.copyFile, fs.copyFileSync, fs.cp,\\ fs.cpSync, fs.createWriteStream, fs.exists, fs.existsSync, fs.fchmod, fs.fchmodSync,\\ fs.fchown, fs.fchownSync, fs.ftruncate, fs.ftruncateSync, fs.lchown, fs.lchownSync,\\ fs.link, fs.linkSync, fs.mkdir, fs.mkdirSync, fs.mkdtemp, fs.mkdtempSync,\\ fs.open, fs.openSync, fs.opendir, fs.opendirSync, fs.read, fs.readFile,\\ fs.readFileSync, fs.readSync, fs.readdir, fs.readdirSync, fs.readlink, fs.readlinkSync,\\ fs.readv, fs.readvSync, fs.rename, fs.renameSync, fs.rm, fs.rmSync,\\ fs.rmdir, fs.rmdirSync, fs.symlink, fs.symlinkSync, fs.truncate, fs.truncateSync,\\ fs.unlink, fs.unlinkSync, fs.write, fs.writeFile, fs.writeFileSync, fs.writeSync,\\ fs.writev, fs.writevSync}\\

./lib/internal/fs/promises.js & \makecell[l]{filehandle.appendFile, filehandle.chmod, filehandle.chown, filehandle.read,\\ filehandle.createReadStream, filehandle.datasync, filehandle.createWriteStream,\\  filehandle.readableWebStream, filehandle.readv, filehandle.truncate, filehandle.write,\\ filehandle.writeFile, filehandle.writev, promises.access, promises.appendFile,\\ promises.chmod, promises.chown, promises.copyFile, promises.cp, promises.link,\\ promises.mkdtemp, promises.mkdir, promises.open, promises.readFile, promises.readdir,\\ promises.readlink, promises.realpath, promises.rename, promises.rm, promises.rmdir,\\ promises.symlink, promises.truncate, promises.unlink, promises.writeFile}\\

./lib/child\_process.js & \makecell[l]{child\_process.exec, child\_process.spawnSync, child\_process.execFile, child\_process.spawn, \\ child\_process.execFileSync, child\_process.execSync, child\_process.fork}\\

./lib/internal/dns/callback\_resolver.js & \makecell[l]{dns.resolve, dns.resolve6, dns.resolveCname, dns.resolveMx, dns.resolveNs, dns.resolveSrv,\\ dns.resolveTxt, dns.reverse}\\

./lib/os.js & \makecell[l]{os.homedir, os.hostname, os.networkInterfaces, os.platform, os.userInfo}\\

./lib/http.js & http.get, http.request\\

./lib/https.js & https.get, https.request\\

./lib/net.js & net.connect, net.write\\

./lib/dgram.js& dgram.connect, dgram.send\\

./lib/\_http\_outgoing.js & request.end, request.write\\

./lib/dns.js & dns.lookup\\

./lib/internal/fs/dir.js & promises.opendir\\

\~ & process.arch, process.env, process.platform, process.versions \\

%\~ & \makecell[l]{process.arch, process.env, process.platform, process.versions}\\

\bottomrule
\end{tabular}
}
\end{table*}

==> tables/Sensitive-Atomic-Operations.tex <==
\begin{table*}[h!t]
    \centering
	\caption{Sensitive Behavior Types}
	\label{tab:Sensitive Atomic Operations}
	\resizebox{\linewidth}{!}{
% 	\begin{tabular*}{\hsize}{@{}@{\extracolsep{\fill}}ll@{}}
	\begin{tabular}{ll}
    	\toprule
		\textbf{Sensitive Behavior Name} & \textbf{Description}   \\
		\midrule
		NETWORK\_OUT &\begin{tabular}[c]{@{}l@{}} Call the API for the network output, including multiple protocols, DNS takeaway and other methods.\end{tabular}   \\      
		NETWORK\_IN & Call the API for network download, including various protocols and methods.  \\ 
		FILE\_READ & \begin{tabular}[c]{@{}l@{}} Call the API for file reading or directory reading, and some APIs need to specify the second parameter as "r".\end{tabular} \\ 
		FILE\_DELETE & Call the API for file deletion.   \\
		FILE\_MODIFY &\begin{tabular}[c]{@{}l@{}} Call the API for file modification, and some APIs need to specify the second parameter as "w" or "a". \end{tabular} \\
		FILE\_CREATE & Call the API for file creation, and some APIs need to specify the second parameter as "w".  \\ 
		CODE\_GENERATION& The calling code executes the API execution string. \\
		SYSTEM\_MESSAGE & Including user information, network interface, user directory, operating system platform, etc. \\
		PROCESS\_MESSAGE & Including the version, environment, platform, etc. of the current process. \\
		PROCESS\_COMMAND\_EXECUTION & Call the command execution API to execute system commands.\\
        PROCESS\_FILE\_EXECUTION & Call file execution API to execute external program.\\
        SERIALIZATION & Call serialization API.\\
% 		PROCESS\_MESSAGE & Including user information, network interface, user directory, operating system platform, etc. \\
% 		SENSITIVE\_FILE\_READ & \begin{tabular}[c]{@{}l@{}}Including reading of system information, ssh information, service information, work plan, \\sensitive directory and other files.\end{tabular} \\
% 		SENSITIVE\_FILE\_DELETE & \begin{tabular}[c]{@{}l@{}}Including the deletion of system information, ssh information, service information, work plans, \\sensitive directories and other files.\end{tabular} \\
% 		SENSITIVE\_FILE\_MODIFY & \begin{tabular}[c]{@{}l@{}}Including modification of system information, ssh information, service information, work plan, \\sensitive directory and other files.\end{tabular} \\
% 		SENSITIVE\_FILE\_CREATE & \begin{tabular}[c]{@{}l@{}}Including the creation of files such as system information, ssh information, service information, \\ work plans, and sensitive directories. \end{tabular}\\
		\hline 
	\end{tabular}
	}
\end{table*}
